Plasmon Fizeau drag in 3D Dirac and Weyl semimetals

There is a need for compact, dynamically tunable nonreciprocal optical elements to enable on-chip-compatible optical isolators and more efficient radiative energy transfer systems. Plasmon Fizeau drag, the drag of electrical current on propagating surface plasmon polaritons, has been proposed to induce nonreciprocal surface modes to enable one-way energy transport. However, relativistic electron drift velocities are required to induce appreciable contrast between the dispersion characteristics of co-propagating and counter-propagating surface plasmon modes. The high electron drift velocity of graphene previously allowed for the experimental demonstration of current-induced nonreciprocity in a two-dimensional (2D) Dirac material. The high electron drift and Fermi velocities in three-dimensional (3D) Dirac materials make them ideal candidates for the effect, however, both the theory of the Fizeau drag effect and its experimental demonstrations in 3D Dirac materials are missing. Here we develop a comprehensive theory of Fizeau drag in DC-biased 3D Weyl semimetals (WSM) or Dirac semimetals (DSM), both under local and non-local approximation and with dissipative losses. We predict that under practical assumptions for loss, Fizeau drag in the DSM Cd$_3$As$_2$ opens windows of pseudo-unidirectional transport. We additionally introduce new figures of merit to rank nonreciprocal plasmonic systems by their potential for directional SPP transport. Further, we propose a new approach for achieving appreciable plasmonic Fizeau drag via optically pumping bulk inversion symmetry breaking WSMs or DSMs.

==> derivation-current.tex <==
\section{Supplemental Note 2: Longitudinal polarizability and optical conductivity in DSM and WSM with current bias }\label{secA2}

\subsection{Nonlocal case}
Here, we derive the dynamical longitudinal polarizability, $\Pi_{\rho,\rho}^u(q,\omega)$, and optical conductivity, $\sigma^u(q,\omega)$, of a bulk Dirac semimetal and Weyl semimetal in a drift current-biased state. As in Supplementary Note~\ref{secA1}, the quasiparticle distribution function is modeled as a combination of the equilibrium distribution, $f^u(\mathbf{ p})$, and a perturbation to the distribution, $ \delta f(\mathbf{ p})$, $f(\mathbf{ p}) = f^u(\mathbf{ p}) + \delta f(\mathbf{ p})$,  assuming an externally applied electric field, $\mathbf{E}= \mathbf{E_0}e^{-i\omega t + i \mathbf{q}\cdot \mathbf{r}}$. In the case of an applied DC current, the equilibrium distribution is a skewed Fermi distribution of the form~\cite{Borgnia2015Quasi-RelativisticGraphene, Dong2021FizeauPlasmonics}:

\begin{equation}
    f^u(\mathbf{ p}) = \frac{1}{e^{(E(\mathbf{p})- \mathbf{u} \cdot \mathbf{p}- \mu^u )/k_BT} +1 },
\end{equation}

\noindent where $E(\mathbf{p})=v|\mathbf{ p}|$. We will express $\nabla_p f^{u}(\mathbf{ p})$  as an integral over the independent energy variable, $\epsilon$ \cite{Borgnia2015Quasi-RelativisticGraphene}
\begin{equation}
    \begin{aligned}
         \nabla_p f^{u}(\mathbf{ p}) = \int d \epsilon \delta(\epsilon - E(\mathbf{p})) (\mathbf{ v_p-u})\frac{\partial f^u(\epsilon, \mathbf{ p})}{\partial \epsilon},
    \end{aligned}
\end{equation}
\noindent where
\begin{equation}
    f^u(\mathbf{ p}) = \frac{1}{e^{(\epsilon - \mathbf{u} \cdot \mathbf{p}- \mu^u )/k_BT} +1 },
\end{equation}
\noindent and note that $ v_\mathbf{ p} = \frac{v^2\mathbf{ p}}{\epsilon}$. From the above equations, we can express the polarizability as

\begin{equation} \label{eq:pol1}
\begin{aligned}
    \Pi^u(\mathbf{ q}, \omega) &= - \frac{g}{\mathcal{V}} \sum_\mathbf{ p} \frac{\mathbf{ q} \cdot \nabla_p f^u(\mathbf{ p})}{\omega- \mathbf{ v_p \cdot  q}}, \\
    & = - \frac{g}{\mathcal{V}} \sum_\mathbf{ p} \int d\epsilon \delta(\epsilon - E(\mathbf{p}))\frac{ v^2\mathbf{ q \cdot  p}- \epsilon\mathbf{ q \cdot u} } {\epsilon\omega - v^2\mathbf{ p}\cdot \mathbf{q} } \frac{\partial f^u(\epsilon, \mathbf{ p})}{\partial \epsilon}. \\
    % & = - \frac{g}{(2\pi\hbar)^3} \int \int dp_x dp_y dp_z \int d\epsilon \delta(\epsilon - E(\mathbf{p}))\frac{ v^2\mathbf{ q \cdot p}- \epsilon\mathbf{ q \cdot u} } {\epsilon\omega - v^2\mathbf{ p}\cdot \mathbf{q}} \frac{\partial f^u(\epsilon, \mathbf{ p})}{\partial \epsilon}   
\end{aligned}
\end{equation}

\noindent To solve Eq.~\ref{eq:pol1}, we will perform a quasi-Lorentz transformation (QLT) with the below transformations for current traveling in the z-direction (this transformation is justified in the main text):

\begin{equation} \label{eq:QLTs-Material}
    \epsilon_0(p)=\gamma\left(\epsilon(p)-up^z\ \right),~
    p_{0}^z=\gamma\left(p^z-\frac{u}{v_F^2}\epsilon(p)\right),~
    p_{0}^x=p^x,~p_{0}^y=p^y,
\end{equation}

\begin{equation} \label{eq:QLTs-EM}
\begin{aligned} 
        \omega_0=\gamma(\omega -u q_z ),~
        q_{0}^z&=\gamma(q^z-\frac{u}{v_F^2}\omega),~
        q_{0}^x=q^x,~
        q_{0}^y=q^y, ~
\end{aligned}
\end{equation}

\begin{equation} \label{eq:QLT-factor}
    \gamma = (1 - u^2/v_F^2)^{-1/2}.
\end{equation}

\noindent Where $\gamma$ is the QLT factor and the subscript ``$0$" represents measurements in the moving frame with velocity $u$ and the subscript ``$u$" represents measurements in the stationary frame (following the notation of \cite{Dong2021FizeauPlasmonics}).

The perturbed density is transformed as

\begin{equation} \label{eq:QLT-density}
    f^{u}(\epsilon) = \frac{1}{e^{(\epsilon- \mathbf{u} \cdot \mathbf{p} - \mu^u )/k_BT}+1} = \frac{1}{e^{(\epsilon_0 -\mu_0)/\gamma k_BT}+1},
\end{equation}

\noindent where we have introduced $\mu_0 =\gamma \mu^u$. The chemical potential must be transformed such that the quasiparticle density, $n$, is conserved: $n_0 = n/\gamma$ ~\cite{Dong2021FizeauPlasmonics}.
The quasiparticle density of a WSM/DSM is $n = \int_0^{\epsilon_F} N(\epsilon) d \epsilon $, where the electron density of states is $N(\epsilon) = \epsilon^2/({2\pi^2\hbar^3v_F^3})$. At 0K we can show that the quasiparticle density is $n =\epsilon_F^3/(6\pi^2\hbar^3v_F^3) $, and thus the carrier density and chemical potential follow the relationship $n\propto \mu^3$~\cite{Hofmann2015PlasmonLiquids}. Therefore, to conserve carrier density the chemical potential must transform as $\mu_0 = \mu/\gamma^{1/3}$ and subsequently $\mu^u = \mu_0/\gamma = \mu/\gamma^{4/3}$.

 Next, note that according to our definition~\cite{Borgnia2015Quasi-RelativisticGraphene}

\begin{equation}
    \frac{\partial f^{u}(\epsilon)}{\partial \epsilon} = \gamma \frac{\partial f^{0}(\epsilon_0)}{\partial \epsilon_0} .
 \end{equation}

 Additionally, the transformation of $\delta(\epsilon - v|p|)$ is found by making use of the delta function identity from quantum field theory~\cite{Peskin1995AnTheory.}, defined using an arbitrary function $g(x)$, the identity is

\begin{equation}
     \delta(g(x)-g(x_0)) = \frac{1}{|g'(x_0)|} \delta(x-x_0).
 \end{equation}
 
\noindent We express the QLT of the energy, $\epsilon_0$, as 
 
 \begin{equation}
     \begin{aligned}
         g(x)  &= \gamma (x - u p(x)), \\
         g'(x)  &= \gamma (1 - u \frac{dp(x)}{dx}),
     \end{aligned}
 \end{equation}

\noindent where $g(x) = \epsilon_0$ and $x = \epsilon$, and via $\epsilon = v|p|$ we know that $p(x) = \epsilon/v = x/v$. Using the delta function identity, we find
% ~\href{https://math.stackexchange.com/questions/4300545/normalization-of-one-particle-states-using-dirac-delta-function}{(Resource)}
  \begin{equation}
  \begin{aligned}
        \delta(\epsilon_0 - v|p_0|) 
        % &= \frac{1}{|\gamma (1 - u \frac{p(x)}{dx})|} \delta(\epsilon - v|p|), \\
      &= \frac{1}{|\gamma (1 - u/v)|} \delta(\epsilon - v|p|), \\
      % &  =\frac{p}{|\gamma (p - u\epsilon/v^2)|} \delta(\epsilon - v|p|), \\
      % &  =\frac{p}{p_0} \delta(\epsilon - v|p|), \\
      &  =\frac{\epsilon_0}{\epsilon} \delta(\epsilon - v|p|). 
  \end{aligned}
 \end{equation}
 
\noindent  Thus,
 \begin{equation} \label{eq:pol2}
\begin{aligned}
    \Pi^{u}(\mathbf{ q}, \omega) 
    % & =  - \frac{g}{(2\pi\hbar)^3} \int \int dp_x dp_y dp_z \int d\epsilon
    % \frac{\epsilon}{\epsilon_0} \delta(\epsilon_0 - v|p_0|) \frac{ v^2\mathbf{ q \cdot p}- \epsilon\mathbf{ q \cdot u} } {\epsilon\omega - v^2\mathbf{ p}\cdot \mathbf{q} } \gamma \frac{\partial f^{0}(\epsilon_0)}{\partial \epsilon_0}. \\
    &= - \frac{g}{\mathcal{V}} \sum_\mathbf{ p} \int d\epsilon
    \frac{\epsilon}{\epsilon_0} \delta(\epsilon_0 - v|p_0|) \frac{ v^2\mathbf{ q \cdot p}- \epsilon\mathbf{ q \cdot u} } {\epsilon\omega - v^2\mathbf{ p}\cdot \mathbf{q} } \gamma \frac{\partial f^{0}(\epsilon_0)}{\partial \epsilon_0}.
\end{aligned}
\end{equation}

\noindent  Under the QLT $ \epsilon\omega -  v_F^2 \mathbf{ p \cdot q} = \epsilon_0\omega_0 - v_F^2 \mathbf{ p_0 \cdot q_0}$ and $v^2 p^z - \epsilon u = v^2 p_{0}^z/\gamma$~\cite{Borgnia2015Quasi-RelativisticGraphene}. 
To extract the longitudinal conductivity, $\Pi^u_{\rho_z,\rho_z}({q}, \omega)=\Pi^u({q}, \omega)$, we again consider the longitudinal case of $\mathbf{ E} || \mathbf{ q} || \mathbf{\hat{z}}$: 
\begin{equation} \label{eq:pol4}
\begin{aligned}
    \Pi^{u}({q}, \omega) 
    % & =  
    % - \frac{g}{(2\pi\hbar)^3} \int \int dp_{x,0} dp_{y,0} dp_0^x    \int d\epsilon_0
    % \frac{\epsilon}{\epsilon_0} \delta(\epsilon_0 - v|p_0|) \frac{ q v_F^2 p_0^x/\gamma} {\epsilon_0\omega_0 - p_0^x v_F^2 q_0} \gamma \frac{\partial f^{0}(\epsilon_0)}{\partial \epsilon_0} \\
    &= - \frac{g}{\mathcal{V}} \sum_\mathbf{p_0} \int d\epsilon_0
    \frac{\epsilon}{\epsilon_0} \delta(\epsilon_0 - v|p_0|) \frac{ q v_F^2 p_0^z/\gamma} {\epsilon_0\omega_0 - p_0^z v_F^2 q_0} \gamma \frac{\partial f^{0}(\epsilon_0)}{\partial \epsilon_0}.
\end{aligned}
\end{equation}

\noindent Solving the $\epsilon_0$ integral over the delta function we get $\epsilon_0 = v|\mathbf{ p_0}|$, leading to

  \begin{equation} \label{eq:pol5}
\begin{aligned}
    \Pi^{u}({q}, \omega) & =  
    % - \frac{g}{(2\pi\hbar)^3} \int \int dp_{x,0} dp_{y,0} dp_0^x  
    % \frac{\epsilon}{\epsilon_0} \frac{ q v_F^2 p_0^x } {\epsilon_0\omega_0 - p_0^x v_F^2 q_0} \frac{\partial f^{0}(\epsilon_0)}{\partial \epsilon_0} . \\
    & =   - \frac{g}{\mathcal{V}} \sum_\mathbf{p_0}
    \frac{\epsilon}{\epsilon_0} \frac{ q v_F^2 p_0^z } {\epsilon_0\omega_0 - p_0^z v_F^2 q_0} \frac{\partial f^{0}(\epsilon_0)}{\partial \epsilon_0} . 
\end{aligned}
\end{equation}

\noindent Note that $ \frac{\epsilon}{\epsilon_0} = \gamma (1+ u p_0^z/\epsilon_0)$, and thus
 
\begin{equation} \label{eq:Fizeau-L-v-NL}
\begin{aligned}
    \Pi^{u}({q}, \omega) & =  
    % - \frac{g}{(2\pi\hbar)^3} \int \int dp_{x,0} dp_{y,0} dp_0^z ~  
    % \gamma (1+ \frac{u p_0^z}{\epsilon_0}) \frac{ q v_F^2 p_0^z } {\epsilon_0\omega_0 - p_0^z v_F^2 q_0}\frac{\partial f^{0}(\epsilon_0)}{\partial \epsilon_0} . \\
    &= - \frac{g}{\mathcal{V}} \sum_\mathbf{p_0} \gamma (1+ \frac{u p_0^z}{\epsilon_0}) \frac{ q v_F^2 p_0^z } {\epsilon_0\omega_0 - p_0^z v_F^2 q_0}\frac{\partial f^{0}(\epsilon_0)}{\partial \epsilon_0} .
\end{aligned}
\end{equation}


\noindent The integral can then be transformed from 3D $p_0$-space to over a constant energy surface $\epsilon_0$ via Eq.~\ref{eq:solid-angle-transform}~\cite{Coleman2015Finite-temperaturePhysics, Borgnia2015Quasi-RelativisticGraphene}

\begin{equation}
\begin{aligned}
    \Pi^{u}({ q}, \omega)  
    % &= - g\int_0^{2\pi} d\phi \int_0^{\pi} \frac{d\theta sin\theta}{4\pi} \int d\epsilon_0 N(\epsilon_0)~ \gamma \left(1+ \frac{u p_0^z}{\epsilon_0} \right)  \frac{ q v_F^2 p_0^z } {\epsilon_0\omega_0 - p_0^z v_F^2 q_0}\frac{\partial f^{0}(\epsilon_0)}{\partial \epsilon_0} . \\
    % & = - g\int_0^{2\pi} d\phi \int_0^{\pi} \frac{d\theta sin\theta}{4\pi} \int d\epsilon_0 N(\epsilon_0)~ \gamma \left(1+ \frac{u p_{0}(\epsilon_0)\cos{\theta}}{\epsilon_0} \right) \frac{ q v_F^2 p_{0}(\epsilon_0)\cos{\theta} } {\epsilon_0\omega_0 - p_{0}(\epsilon_0)\cos{\theta} v_F^2 q_0}. \\
    & = - g\int_0^{2\pi} d\phi \int_0^{\pi} \frac{d\theta sin\theta}{4\pi} \int d\epsilon_0 N(\epsilon_0)~ 
    \gamma \left(1+ \frac{u p_{0}\cos{\theta}}{\epsilon_0} \right) \frac{ q v_F^2 p_{0}\cos{\theta} } {\epsilon_0\omega_0 - p_{0}\cos{\theta} v_F^2 q_0}
    \frac{\partial f^{0}(\epsilon_0)}{\partial \epsilon_0}.
\end{aligned}
\end{equation}

\noindent  This can be evaluated for low temperature $kT \ll \mu$ using ${\partial f^{0}(\epsilon_0)}/{\partial \epsilon_0} \approx - \delta \left( \epsilon_0 - \mu_0 \right) $ ~\citep{Peskin1995AnTheory.,Borgnia2015Quasi-RelativisticGraphene}

\begin{equation}
\begin{aligned}
    \Pi^{u}({ q}, \omega) 
    % & = g N(\mu_0) \int_0^{2\pi} d\phi \int_0^{\pi} \frac{d\theta sin\theta}{4\pi} ~ 
    % \gamma \left(1+ \frac{u p_0^z}{\mu_0} \right) \frac{ q v_F^2 p_0^z} {\mu_0\omega_0 - p_0^z v_F^2 q_0}, \\
    % & = g N(\mu_0) \int_0^{2\pi} d\phi \int_0^{\pi} \frac{d\theta sin\theta}{4\pi} ~ \gamma \left(1+ \frac{u p_{0}(\mu_0)\cos{\theta}}{\mu_0} \right) \frac{ q v_F^2 p_{0}(\mu_0)\cos{\theta} } {\mu_0\omega_0 - p_{0}(\mu_0)\cos{\theta} v_F^2 q_0}.
    & = g N(\mu_0) \int_0^{2\pi} d\phi \int_0^{\pi} \frac{d\theta sin\theta}{4\pi} ~ \gamma \left(1+ \frac{u p_{0}\cos{\theta}}{\mu_0} \right) \frac{ q v_F^2 p_{0}\cos{\theta} } {\mu_0\omega_0 - p_{0}\cos{\theta} v_F^2 q_0}.
\end{aligned}
\end{equation}

\noindent Note that $\frac{1}{v_F} = \frac{p_{0}(\mu_0)}{\mu_0}$, and thus


\begin{equation}
\begin{aligned}
    \Pi^{u}({ q}, \omega) & = g N(\mu_0) 2\pi \int_0^{\pi} \frac{d\theta sin\theta}{4\pi} ~ 
    \gamma \left(1+ \frac{u\cos{\theta}}{v_F} \right) \frac{ v_F q\cos{\theta} } {\omega_0 - v_F q_0 \cos{\theta} }. 
\end{aligned}
\end{equation}

\noindent Let $a=\cos\theta$ , $\frac{da}{d\theta} = -\sin\theta$, and $d\theta \sin\theta = -da$:
\begin{equation}
\begin{aligned}
    \Pi^{u}({q}, \omega) & = g N(\mu_0) \frac{\gamma}{2} \int_1^{-1} -da ~ 
    \left( 1+ \frac{u a}{v_F} \right) \frac{ v_F q a } {\omega_0 - v_F q_0 a }, \\
     & = -g N(\mu_0) \frac{1}{2} 
     \frac{q \gamma (q_0 v_F^2 +u\omega_0)}{q_0^3 v_F^3} 
     \left( \omega_0 \ln \left( \frac{\omega_0 - q_0 v_F}{\omega_0 + q_0 v_F}\right) +2 q_0 v_F
    \right), \\
    & = - g N(\mu_0) 
     \frac{q \gamma (q_0 +\frac{u}{v_F^2}\omega_0)}{q_0^2} 
     \left( \frac{\omega_0}{2 q_0 v_F} \ln \left( \frac{\omega_0 - q_0 v_F}{\omega_0 + q_0 v_F}\right) +1
    \right), \\
    & = - g N(\mu_0) 
     \frac{q^2}{q_0^2} 
     \left( \frac{\omega_0}{2 q_0 v_F} \ln \left( \frac{\omega_0 - q_0 v_F}{\omega_0 + q_0 v_F}\right) +1
    \right) .
\end{aligned}
\end{equation}


\noindent The longitudinal polarizability is converted to longitudinal optical conductivity as follows:

\begin{equation} \label{eq:Fizeau-cond}
\begin{aligned}
    {\mbox{Im}\sigma^u_{zz}} (q,\omega) & = \frac{ie^2\omega}{q^2} \mbox{Re}\Pi^u (q, \omega), \\ 
    % & = -\frac{ie^2\omega}{q^2} g N(\mu_0) \left( 
    %  \frac{q^2}{q_0^2} 
    %  \left( \frac{\omega_0}{2 q_0 v_F} \ln \left( \frac{\omega_0 - q_0 v_F}{\omega_0 + q_0 v_F}\right) +1
    % \right)  \right) \\ 
    & = -\frac{ie^2\omega}{q_0^2} g N(\mu_0) 
     \left( \frac{\omega_0}{2 q_0 v_F} \ln \left( \frac{\omega_0 - q_0 v_F}{\omega_0 + q_0 v_F}\right) +1
    \right) . \\ 
\end{aligned}
\end{equation}
\noindent Comparing Eq.~\ref{eq:Fizeau-cond} to Eq.~\ref{eq:Normal-cond-Im}, we have shown that the longitudinal optical conductivity is transformed under Fizeau drag as:

\begin{equation} \label{eq:Fizeau-transform-result}
\begin{aligned} 
        \sigma_{zz}^{u} (\omega,q,\mu)
        &=  \frac{\omega}{\omega_0}\sigma_{zz}(\omega_0,q_0,\mu_0), \\
\end{aligned}
\end{equation}
where
\begin{equation} \label{eq:QLTs}
\begin{aligned} 
        \omega_0=\gamma(\omega -u q_z ),~
        q_{z,0}&=\gamma(q_z-\frac{u}{v_F^2}\omega),~
        q_{x,0}=q_x,~
        q_{y,0}=q_y, ~
        \mu_0 = \frac{\mu}{\gamma^{1/3}}.
\end{aligned}
\end{equation}


\subsection{Local case }
For thoroughness and comparison, we show that the same Fizeau drag derivation can be performed for the local case, making use of Taylor series expansion around $q_0 \rightarrow 0$ starting from equation~\ref{eq:Fizeau-L-v-NL}:

\begin{equation} \label{eq:polar-xx}
\begin{aligned}
    \frac{ q v_F^2 p_0^z} {\epsilon_0\omega_0 - p_0^z v_F^2 q_0} = \frac{ q v_F^2 p_0^z} {\epsilon_0\omega_0} + \frac{ qq_0 v_F^4 (p_0^z)^2} {\epsilon_0^2\omega_0^2} + O[q]^2 \\ 
\end{aligned}
\end{equation}

\begin{equation} \label{eq:polar-xx-b}
\begin{aligned}
    (1+ \frac{u p_0^z}{\epsilon_0})\frac{ q v_F^2 p_0^z} {\epsilon_0\omega_0 - p^x_0 v_F^2 q_0} &\approx 
    (1+ \frac{u p_0^z}{\epsilon_0}) \left( \frac{ q v_F^2 p_0^z} {\epsilon_0\omega_0} + \frac{ qq_0 v_F^4 (p_0^z)^2} {\epsilon_0^2 \omega_0^2} \right) \\
    &\approx \frac{ q u v_F^2 (p_0^z)^2} {\epsilon^2_0 \omega_0} + \frac{ q q_0 v_F^4 (p_0^z)^2} {\epsilon_0^2 \omega_0^2} \\ 
    % &= \frac{ q v_F^2 p_0^z^2}{\epsilon^2_0\omega^2_0} ( u{\omega_0} + {q_0 v_F^2 } ) \\ 
    %  &= \frac{ q v_F^4 p_0^z^2}{\epsilon^2_0\omega^2_0} ( \frac{u{\omega_0}}{v_F^2} + {q_0} ) \\ 
    %  &= \frac{ q v_F^4 p_0^z^2}{\epsilon^2_0\omega^2_0} \frac{q}{\gamma} \\ 
     &= \frac{ q^2 v_F^4 (p_0^z)^2}{\epsilon^2_0 \omega^2_0} \frac{1}{\gamma} . \\ 
\end{aligned}
\end{equation}
\noindent  Thus,
 \begin{equation} \label{eq:pol11}
\begin{aligned}
    \Pi^u({q}, \omega) & \approx  - \frac{g}{\mathcal{V}} \sum_\mathbf{p_0} ~  
    \frac{ q^2 v_F^4 (p_0^z)^2}{\epsilon^2_0\omega^2_0} \frac{\partial f^{0}(\epsilon_0)}{\partial \epsilon_0} .
\end{aligned}
\end{equation}
\noindent  The integral can then be transformed from 3-dimensional $p$-space to over a constant energy surface via Eq.~\ref{eq:solid-angle-transform} 

\begin{equation} \label{eq:pol8}
\begin{aligned}
    \Pi^u({ q}, \omega) & = - g\int_0^{2\pi} d\phi \int_0^{\pi} \frac{d\theta sin\theta}{4\pi} \int d\epsilon N(\epsilon)~  
    \frac{ q^2 v_F^4 (p_{0}(\epsilon_0)\cos{\theta})^2}{\epsilon^2_0\omega^2_0} \frac{\partial f^{0}(\epsilon_0)}{\partial \epsilon_0} .
\end{aligned}
\end{equation}

\noindent  As for the nonlocal case, this is evaluated for low-temperature $kT \ll \mu$ using ${\partial f^{0}(\epsilon_0)}/{\partial \epsilon_0} \approx - \delta \left( \epsilon_0 - \mu_0 \right) $

\begin{equation} \label{eq:pol10}
\begin{aligned}
    \Pi^u({q}, \omega) & =  g\frac{ q^2 v_F^2 }{\omega^2_0} N(\mu_0)\int_0^{2\pi} d\phi \int_0^{\pi} \frac{d\theta }{4\pi}\sin{\theta}\cos^2{\theta} , \\
    & =   \frac{1}{3} N(\mu_0)g  
    \frac{ q^2 v_F^2 }{\omega^2_0} ,  \\
    & = \frac{1}{3} \frac{g\mu_0^2}{2\pi^2\hbar^3v_F}~  
    \frac{ q^2}{\omega^2_0} .
\end{aligned}
\end{equation}

\noindent The longitudinal polarizability is converted to longitudinal optical conductivity 

\begin{equation}
\begin{aligned}
    \sigma^u_{zz}(q,\omega) &= \frac{\omega}{\omega_0}  \frac{i e^2 g \mu_0^2}{6\pi^2\hbar^3\omega_0v_F}, \\
    &= \frac{\omega}{\gamma(\omega-uq)}  \frac{i e^2 g \mu_0^2}{6\pi^2\hbar^3v_F\cdot\gamma(\omega-uq)}.
\end{aligned}   
\end{equation}

\noindent When compared to the non-current carrying case, it is clear that the longitudinal optical conductivity is transformed again following equations ~\ref{eq:Fizeau-transform-result} and~\ref{eq:QLTs}. 

\newpage
In Suppl. Fig.~\ref{fig:NL-L_RPA-SPP-comparisons}(a-d) we plot the SPP dispersion for lossless Cd$_3$As$_2$ for increasing current biases using the local Drude, Eq.~\ref{eq:pol-SC-local}, nonlocal Drude, Eq.~\ref{eq:pol-normal}, and RPA, Eq.~\ref{eq:pol-RPA}, dielectric models. The RPA and nonlocal Drude models closely match, while the local Drude model does not align with either result. With increased carrier velocity, the local and nonlocal optical models increasingly diverge, resulting in vastly different plasmon frequencies, where the local model overestimates the magnitude of Fizeau shift. This emphasizes the importance of accounting for nonlocality in Fizeau drag calculations.

The nonlocal predictions for Fizeau drag differs notably from the prediction of truly unidirectional SPP transport which can be made when invoking the non-realistic local Drude mode. The local Drude model predicts that the counter-propagating mode will never bend upward to compete with the co-propagating mode, facilitating unidirectionality. 
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/L-v-NL-RPA-SPPs.jpg}
    \caption{The SPP dispersion for Cd$_3$As$_2$ ($v_F=1\times10^{6}$, $\epsilon_F = 0.15$ eV, and $g=4$) for the local Drude~\cite{Kotov2016DielectricFilms}, Eq.~\ref{eq:pol-SC-local}, nonlocal Drude, Eq.~\ref{eq:pol-normal}, and the RPA dielectric model presented in Ref.~\cite{Thakur2017DynamicalSystems,Thakur2018DynamicSemimetals}, Eq.~\ref{eq:pol-RPA}, for the (a) unbiased case and (b) $u=0.1v_F$, (c) $u=0.3v_F$, and (d) $u=0.5v_F$. }
    \label{fig:NL-L_RPA-SPP-comparisons}
\end{figure}
\newpage
\section{Supplemental Note 3: Complex-q solving method}\label{sec:A3}

All the SPP mode solutions shown in this manuscript have been found by searching over a complex $q = \mbox{Re}(q) + \mbox{Im}(q)$ space as shown in Suppl. Fig.~\ref{fig:complex-q-space}. The solutions corresponding to lossy non-propagating modes, with $\mbox{Re}(q)/\mbox{Im}(q)<1$, are included in the main figures, while the solutions representing gain, $\mbox{Re}(q)/\mbox{Im}(q)>1$, are assumed to be unphysical~\cite{Gangaraj2022DriftingPhotonics}, but are included in  Supplementary Fig.~\ref{fig:complex-q-space} in black. The SPP dispersion for Cd$_3$As$_2$ without any Fizeau drag is shown in Supplementary Fig.~\ref{fig:noFizeau-lossy}.

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{figures/complex-q-space-suppl.jpg}
    \caption{\textbf{Complex q-space solution for increasing loss. }The equifrequency complex wavevector solution space for $\omega =0.337\epsilon_F$ for (a) $\tau = 2.1\times 10^{-10}s$, (b) $\tau = 2.1\times 10^{-11}$s, (c) $\tau = 2.1\times 10^{-12}$s and the corresponding SPP dispersion for each in (d), (e), and (f) respectively. The solid line represented the $\mbox{Re}(q)$ solution and the dashed represented the $\mbox{Im}(q)$ solution. The black corresponds to the solution representing gain, $\mbox{Re}(q)/\mbox{Im}(q)>1$.The same Cd$_3$As$_2$ parameters are used as in Fig.~\ref{fig:lossy-result}.}
    \label{fig:complex-q-space}
\end{figure}
In Suppl. Fig.~\ref{fig:noFizeau-lossy}(a-c) we show the SPP dispersion for Cd$_3$As$_2$ for decreasing scattering period from $\tau=2.1\times 10^{-10}$s to $2.1\times 10^{-12}$s.
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/lossy_SPP_noFizeauDrag.jpg}
    \caption{The SPP dispersion for Cd$_3$As$_2$ ($v_F=1\times10^{6}$, $\epsilon_F = 0.15$ eV, and $g=4$) for the nonlocal Drude model derived in Eq.~\ref{eq:pol-normal} under no DC-bias in the (a) $\tau=2.1\times 10^{-10}$, (b) $\tau=2.1\times 10^{-11}$ and (c) $\tau=2.1\times 10^{-12}$ case. }
    \label{fig:noFizeau-lossy}
\end{figure}
\newpage
\section{Supplementary Note 4: Comparison to graphene Fizeau drag}\label{sec:A4}

Here we plot the SPP dispersion for Fizeau drag in graphene using the derivations presented in Ref.~\cite{Dong2021FizeauPlasmonics} for the air, Suppl. Fig~\ref{fig:graphene}(a), and hBN encapsulated, Suppl. Fig~\ref{fig:graphene}(b), cases. These are shown alongside the SPP dispersion for the 3D DSM Cd$_3$As$_2$. In all the panels, the dispersion characteristics have been calculated by using nonlocal optical models in the lossless case.
\begin{figure} [ht]
    \centering
    \includegraphics[width=1\linewidth]{figures/graphene-comparison.jpg}
    \caption{The SPP dispersion for Fizeau drag in (a) Graphene in air (b) Graphene encapsulated in hBN and (c) the 3D DSM Cd$_3$As$_2$. The graphene is modeled following the equations in Ref.~\cite{Dong2021FizeauPlasmonics}, using $n=2.88\times 10^{12}$, $v_F=1\times 10^6$ms$^{-1}$, $E_F=198$ meV. The hBN is modeled using the parameters from Ref.~\cite{Ni_McLeod_Sun_Wang_Xiong_Post_Sunku_Jiang_Hone_Dean_2018}. The Cd$_3$As$_2$ is modeled with the same parameters as in Fig.~\ref{fig:fizeauResults}.}
    \label{fig:graphene}
\end{figure}




% \begin{equation}
% \begin{aligned}
%     {\sigma_{zz}} (q,\omega) & = \frac{1}{6} \frac{ie^2g\mu^2}{\pi^2\hbar^3\omega v_F} 
% \end{aligned}
% \end{equation}

% \begin{equation}
% \begin{aligned} 
%         \sigma_{zz}^{u} (\omega,q,\mu)
%         &=  \frac{\omega}{\omega_0}\sigma_{zz}(\omega_0,q_0,\mu_0) \\
%         \omega_0=\gamma(\omega -u q_z ),~
%         q_0^z&=\gamma(q^z-\frac{u}{v_F^2}\omega),~
%         q_0^x=q^x,~
%         q_0^y=q^y, ~
%         \mu_0 = \frac{\mu}{\gamma^{1/3}}
% \end{aligned}
% \end{equation}

% Accounting for loss, this becomes

% \subsection{Local case with loss}

% \begin{equation} 
% \begin{aligned}
%     \Pi_{\tau}(\mathbf{ q}, \omega) 
%     & = \frac{(1+i/\omega\tau)\Pi(q,\omega+i/\tau)}{1+(i/\omega\tau)\Pi(q,\omega+i/\tau)/\Pi(q,0)}  \\
%     & = (1+i/\omega\tau)\Pi(q,\omega+i/\tau) \\
%     &=  (1+i/\omega\tau) \frac{1}{6} \frac{g\mu_0^2}{\pi^2\hbar^3v_F}~  
% \frac{ q^2}{\omega^2_0}  \\
% &=  (\omega+i/\tau)\frac{1}{\omega} \frac{1}{6} \frac{g\mu_0^2}{\pi^2\hbar^3v_F}~  
% \frac{ q^2}{\gamma^2(\omega+i/\tau -u q_z )^2}  \\
% \end{aligned}
% \end{equation}

% \begin{equation}
% \begin{aligned}
%     \sigma^u_{zz}(q,\omega) 
%     % &= \frac{i e^2 \omega}{q^2} (\omega+i/\tau)\frac{1}{\omega} \frac{1}{6} \frac{g\mu_0^2}{\pi^2\hbar^3v_F}~  \frac{ q^2}{\gamma^2(\omega+i/\tau -u q_z )^2}\\
% &= \frac{\omega+i/\tau}{\gamma(\omega+i/\tau -u q_z )}\frac{1}{6} \frac{i e^2g\mu_0^2}{\pi^2\hbar^3v_F\gamma(\omega+i/\tau -u q_z )}~\\
% \end{aligned}   
% \end{equation}

